Fast image reverse filters through fixed point and gradient descent acceleration

In this paper, we study the problem of reverse image filtering. An image filter denoted g(.), which is available as a black box, produces an observation b = g(x) when provided with an input x. The problem is to estimate the original input signal x from the black box filter g(.) and the observation b. We study and re-develop state-of-the-art methods from two points of view, fixed point iteration and gradient descent. We also explore the application of acceleration techniques for the two types of iterations. Through extensive experiments and comparison, we show that acceleration methods for both fixed point iteration and gradient descent help to speed up the convergence of state-of-the-art methods.

==> supplementary_material.tex <==

\newpage
\setcounter{section}{0}
\huge{\textbf{Supplementary material}}

\section{Adaptive Manifolds for Real-Time High-Dimensional Filtering}


\begin{figure}[h!]
    \centering
    \begin{subfigure}{0.24\linewidth}
        \includegraphics[trim=0 0 0 0, clip,width=\linewidth]{New_images/AMF/PSNR_T_AFP_AMF.eps}
        \caption{T-Method}
        \label{fig:T_APF_PSNR2}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}
        \includegraphics[trim=0 0 0 0, clip,width=\linewidth]{New_images/AMF/PSNR_TDA_AFP_AMF.eps}
        \caption{TDA-Method}
        \label{fig:TDA_AFP_PSNR2}
    \end{subfigure}
        \begin{subfigure}{0.24\linewidth}
        \includegraphics[trim=0 0 0 0, clip,width=\linewidth]{New_images/AMF/PSNR_P_AFP_AMF.eps}
        \caption{P-Method}
        \label{fig:P_AFP_PSNR2}
    \end{subfigure}
            \begin{subfigure}{0.24\linewidth}
        \includegraphics[trim=0 0 0 0, clip,width=\linewidth]{New_images/AMF/PSNR_P2_AFP_AMF.eps}
        \caption{New P-Method}
        \label{fig:P2_AFP_PSNR2}
    \end{subfigure}

    \caption{Reversing an AMF filter with different reverse filtering methods and accelerated fixed point iteration.}
    \label{fig:AFP_PSNR2}
\end{figure}    



\begin{figure}[h!]
    \centering
    \begin{subfigure}{0.24\linewidth}
        \includegraphics[trim=0 0 0 0, clip,width=\linewidth]{New_images/AMF/PSNR_T_AGD_AMF.eps}
        \caption{T-Method}
        \label{fig:T_AGD_PSNR2}
    \end{subfigure}
    \begin{subfigure}{0.24\linewidth}
        \includegraphics[trim=0 0 0 0, clip,width=\linewidth]{New_images/AMF/PSNR_TDA_AGD_AMF.eps}
        \caption{TDA-Method}
        \label{fig:T_AGD_PSNR2}
    \end{subfigure}
        \begin{subfigure}{0.24\linewidth}
        \includegraphics[trim=0 0 0 0, clip,width=\linewidth]{New_images/AMF/PSNR_P_AGD_AMF.eps}
        \caption{P-Method}
        \label{fig:T_AGD_PSNR2}
    \end{subfigure}
            \begin{subfigure}{0.24\linewidth}
        \includegraphics[trim=0 0 0 0, clip,width=\linewidth]{New_images/AMF/PSNR_P2_AGD_AMF.eps}
        \caption{p-Method}
        \label{fig:T_AGD_PSNR2}
    \end{subfigure}

    \caption{Reversing an AMF with different reverse filtering methods and accelerated gradient descent.}
    \label{fig:AGD_PSNR2}
\end{figure}    

\begin{figure}[h!]
    \centering
    \begin{subfigure}{0.24\linewidth}
        \includegraphics[trim=0 3cm 0 0, clip,width=\linewidth]{New_images/AMF/AMF_GT.png}
        \caption{Ground Truth}
    \end{subfigure}
        \begin{subfigure}{0.24\linewidth}
        \includegraphics[trim=0 3cm 0 0, clip,width=\linewidth]{New_images/AMF/AMF_Input.png}
        \caption{Input image}
    \end{subfigure}
        \begin{subfigure}{0.24\linewidth}
        \includegraphics[trim=0 3cm 0 0, clip,width=\linewidth]{New_images/AMF/AMF_T.png}
        \caption{T-method}
    \end{subfigure}
        \begin{subfigure}{0.24\linewidth}
        \includegraphics[trim=0 3cm 0 0, clip,width=\linewidth]{New_images/AMF/AMF_TDA.png}
        \caption{TDA-method}
    \end{subfigure}
        \begin{subfigure}{0.24\linewidth}
        \includegraphics[trim=0 3cm 0 0, clip,width=\linewidth]{New_images/AMF/AMF_P.png}
        \caption{P-method}
    \end{subfigure}
            \begin{subfigure}{0.24\linewidth}
        \includegraphics[trim=0 3cm 0 0, clip,width=\linewidth]{New_images/AMF/AMF_P2.png}
        \caption{p-method}
    \end{subfigure}
   \begin{subfigure}{0.24\linewidth}
        \includegraphics[trim=0 3cm 0 0, clip,width=\linewidth]{New_images/AMF/AMF_T_AA.png}
        \caption{T+AFP}
    \end{subfigure}
     \begin{subfigure}{0.24\linewidth}
        \includegraphics[trim=0 3cm 0 0, clip,width=\linewidth]{New_images/AMF/AMF_T_SGDR.png}
        \caption{T+AGD}
    \end{subfigure}
    
    \caption{Reversing an AMF filter with different reverse filtering methods. a) Ground truth image, b) Input blurred image, c) d) e) f) results using the classic T, TDA, P and p methods respectively without modification. g) Best result applying AFP which was achieved by the T+AA method, h) best result applying AGD achieved by T+SGDR.}
    \label{fig:GF_visual}
\end{figure}




